Language Model Beats Diffusion -- Tokenizer is Key to Visual Generation

While Large Language Models (LLMs) are the dominant models for generative tasks in language, they do not perform as well as diffusion models on image and video generation. To effectively use LLMs for visual generation, one crucial component is the visual tokenizer that maps pixel-space inputs to discrete tokens appropriate for LLM learning. In this paper, we introduce MAGVIT-v2, a video tokenizer designed to generate concise and expressive tokens for both videos and images using a common token vocabulary. Equipped with this new tokenizer, we show that LLMs outperform diffusion models on standard image and video generation benchmarks including ImageNet and Kinetics. In addition, we demonstrate that our tokenizer surpasses the previously top-performing video tokenizer on two more tasks: (1) video compression comparable to the next-generation video codec (VCC) according to human evaluations, and (2) learning effective representations for action recognition tasks.

==> sections/method_bk.tex <==
Our goal is to develop a visual tokenizer which can compress images or videos into a set of discrete tokens which are amenable for generative modeling via language models. To that end, we build on MAGVIT~\citep{yu2022magvit}, and focus on two key components of our \modelname: a lookup-free quantizer and an improved model architecture.  

\subsection{Lookup-Free Quantizer}
Visual tokenizers are autoencoders trained via minimizing the reconstruction error~\citep{van2017neural}. Although the community has made great progress in developing VQ-VAEs, the relationship between improvements in the reconstruction quality and subsequent generation quality is not well understood. For example, one way to improve the reconstruction quality is by simply increasing the vocabulary size. However, as shown in Fig.~\ref{fig:motivation}, although the reconstruction FID (right $y$-axis, lower value is better) decreases as we increase the vocabulary size, the generation quality via LM does not monotonically improve. Indeed, current visual generative models~\citep{esser2021taming,villegas2022phenaki} use vocabulary sizes between $2^{10}$ and $2^{13}$, which are significantly smaller than the vocabulary sizes used by state-of-the-art language models (over $2^{17}$). 

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-4mm}
    \centering
    \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{curve.pdf}
    \vspace{-4mm}
    \caption{\textbf{Reconstruction and generation quality curves} when scaling the vocabulary size with Vector Quantization (VQ) and Lookup-Free Quantization (LFQ). 
    }
    \label{fig:motivation}
    \vspace{-4mm}
\end{wrapfigure}

\vspace{-4mm}

\paragraph{Lookup-Free Quantization (\quantizername{}).} A simple trick for training a larger codebook involves decreasing the code embedding dimension when increasing the vocabulary size. 
This trick captures the intuition of limiting the representational capacity of individual words which in turn facilitates the learning of the word distribution. 

Motivated by this observation, we reduce the VQ-VAE codebook's embedding dimension to zero. Formally, the codebook $\rmC \in \sR^{K \times d}$ is replaced with an integer set $\sC$ where $|\sC| = K$. Recall that in VQ-VAE models, the quantizer must lookup all $K\times d$ codebook embeddings, where $d$ is typically $256$, when computing the closet codebook entry to the encoder output. This new design eliminates the need for such embedding lookup entirely hence we call it \emph{lookup-free quantization (\quantizername{})}.

We found that \quantizername{} can grow the vocabulary size in a way benefiting the generation quality of language models. As shown by the blue curves in \cref{fig:motivation}, both reconstruction and generation consistently improves as the vocabulary size increases -- a property not observed in current VQ-VAE methods.

While various \quantizername{} methods are available, this paper discusses a straightforward variant that assumes independent codebook dimensions and binary outputs. Specifically, the latent space of \quantizername{} is decomposed as the Cartesian product of single-dimensional variables, as $\sC = \bigtimes_{i=1}^{\log_2{K}}C_i$.

Given a feature vector $\rvx \in \sR^{\log_2{K}}$, each dimension of the quantized representation $\rvq(\rvx)$ is obtained from:
\begin{equation}
\vspace{-1mm}
    \ervq(\ervx_i) = C_{i, j}, \text{ where } j = \argmin_k |\ervx_i - C_{i, k}|,
\end{equation}
%Depending on the values in $C_i$, we have various ways to compute the $\argmin$. However,
where $C_{i, j}$ is the $j$-th value in $C_i$.
With $C_i = \{-1, 1\}$, the $\argmin$ can be computed by a sign function as 
\begin{equation}
\vspace{-1mm}
    \ervq(\ervx_i) = \sign(x_i) = -\1\{x_i \le 0\} + \1\{x_i > 0\}.
\end{equation}

The token index for an image patch is given by:
\begin{equation}
\vspace{-2mm}
\mathit{Id}(\rvx) = \sum_{i=1}^{\log_2{K}} \argmin_k \|\ervx_i - C_{i, k}\| \prod_{b=0}^{i-1} |C_b| = \sum_{i=1}^{\log_2{K}} 2^{i-1} \1\{x_i > 0\}, \label{eq:tokenid}
\end{equation}
where $|C_0|=1$ sets the virtual basis.

We add an entropy penalty during training to encourage codebook utilization:
\begin{align}
    \gL_\mathit{entropy} &= \E[H(\rvq(\rvx))] - H[\E(\rvq(\rvx))].
\end{align}
This penalty is inspired by a similar loss used in image VQGAN model~\citep{chang2022maskgit}, which is also found in entropy-based clustering~\citep{jansen2020coincidence}. In \quantizername{}, given the independence among dimensions, we rewrite $H(\rvq(\rvx)) = \sum_{i=1}^{\log_2{K}} H(\ervq (\ervx_i))$ .
The $H[\E(\rvq(\rvx))]$ term can be approximated with sub-groups of dimensions for $K>2^{18}$ where direct estimation is memory bound. 



We note that there are various other variants of \quantizername{}, \eg, opting for the multivariant over the binary codebook $C_i$ or employing \citet{agustsson2019generative}.
%or using mutivaint codebook instead of the binary code. 
As the first paper to introduce this concept, we focus on the simplest form with independent binary dimensions, which shows promising improvements. Other \quantizername{} methods merit further research. 



\subsection{Visual Tokenizer Model Improvement}\label{sec:tokenizer_improvement}
\begin{figure}[tp]
\vspace{-4mm}
    \centering
    \begin{subfigure}{1\textwidth} % no visible
    \refstepcounter{subfigure}\label{fig:arch:a}
    \refstepcounter{subfigure}\label{fig:arch:b}
    \refstepcounter{subfigure}\label{fig:arch:c}
    \end{subfigure}%
    \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{causal_arch}
    \vspace{-4mm}
    \caption{\textbf{Causal tokenizer architecture comparison}. \textbf{(a)} C-ViViT. \textbf{(b)} Hybrid of C-ViViT and MAGVIT, where the 3D CNN processes blocks of 4 frames, connected by a causal transformer.
    \textbf{(c)} \modelname{}: causal 3D CNN using causal convolutions in the temporal dimension. The decoders, which are omitted from the figure, employ an architecture that is symmetric to the encoder.
    }
    \label{fig:arch}
    \vspace{-4mm}
\end{figure}

\vspace{-2mm}
\paragraph{Joint image-video tokenization.} Ideally we would like to have a single tokenizer which can tokenize images or videos using a shared codebook. Most prior work has focused on image or video-specific tokenizers, with C-ViViT~\citep{villegas2022phenaki} being a notable exception. C-ViViT (\cref{fig:arch:a}) consists of spatial and causal temporal transformer blocks. Although this approach is effective, it suffers from two limitations. First, positional embeddings in transformer make it difficult to tokenize spatial resolutions that were not seen during training. Second, empirically we found that 3D CNNs perform better than spatial transformer.

We explore two different encoder designs for processing images and videos. A hybrid encoder (\cref{fig:arch:b}) replaces the spatial transformer of C-ViViT with MAGVIT-style 3D encoder. Assuming a temporal compression ratio of $4$, a 3D CNN processes blocks of 4 frames followed by a causal transformer. In \modelname{} (\cref{fig:arch:c}), we replace the 3D CNNs with temporally causal 3D CNNs. A regular 3D convolution layer with kernel size $(k_t, k_h, k_w)$ pads the input temporally with $\lfloor\frac{k_t-1}{2}\rfloor$ frames before and $\lfloor\frac{k_t}{2}\rfloor$ frames after the input. In contrast, a causal 3D convolution only pads with $k_t - 1$ frames before the input, and no frames after, so each output frame depends only on previous input frames. Consequently, the first frame is always independent of other frames, allowing the model to tokenize single images. Temporal subsampling with stride $k$ downsamples the input by $k$ times by mapping frames $1 + k \cdot t$ in the input to frame $1 + t$ in the output. After regular $k$ times upsampling, we drop the first $k - 1$ resulting frames, which maps $1 + t$ input frames to $1 + k \cdot t$ output frames. As shown in Table \ref{tab:ablation_arch}, we empirically evaluate these designs and find that the causal 3D CNN performs best.

\vspace{-4mm}
\paragraph{Architecture modifications.} 

In addition to using causal 3D CNN layers, we made several other architectural modifications to improve upon the MAGVIT model.
First, we replaced the encoder downsample layers from average pooling to strided convolutions in order to leverage learned kernels. We also replaced the decoder upsample layers from nearest neighbor resizing followed by convolution with a depth-to-space operator. Second, we deferred temporal downsampling from the first few encoder blocks to the later ones. Additionally, the downsampling layer in the discriminator now uses 3D blur pooling~\citep{zhang2019making} to encourage shift invariance. Finally, we added an adaptive group normalization layer before the residual blocks at each resolution in the decoder. The quantized latents are passed to these layers as a control signal, following StyleGAN~\citep{karras2019style}. 
% \agrim{I am not sure what this passes line means but I have kept it here}


\vspace{-4mm}
\paragraph{Token factorization for efficient prediction.}
The output tokens can be fed into language models to generate videos. To assist smaller transformers predicting in a large codebook, we can factorize the \quantizername{} token's latent space into equal subspaces. For instance, rather than predicting using a codebook of size $2^{18}$, we can predict in two concatenated codebooks, each of size $2^9$. We embed each subspace token separately and use their embedding summation as the token embedding for the transformer input. For the output layer with weight tying~\citep{press2017using}, we use the embedding matrix for each subspace to obtain logits by seperate prediction heads. 


==> tables/generation_bk2.tex <==
\begin{table}[p]
\centering
\caption{\textbf{Video and image generation results}. 
\emph{Method types}: AutoRegressive Language Model (ARLM), Masked Language Model (MLM), Generative Adversarial Network (GAN), continuous Diffusion (Diff.). 
\emph{Latent types}: \quantizerfullname{} (\quantizername{}), Vector Quantization (VQ), Variational AutoEncoder (VAE), Discrete Cosine Transformation (DCT). guidance indicates the classifier-free diffusion guidance.
We report the bits per pixel (bpp) of the representation used in each latent-space model.
$^*$ indicates usage of extra training data.
}
\label{tab:generation}
\vspace{-2mm}
\begin{subtable}{\linewidth}
\caption{Frame prediction on Kinetics-600 and class-conditional generation on UCF-101.}
\label{tab:gen_k600_full}
\vspace{-2mm}
\resizebox{\linewidth}{!}{%
\centering
\begin{tabular}{@{}l@{\hspace{5pt}}l@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{3pt}}c@{\hspace{5pt}}c@{}}
\toprule
Type & Method   & K600 FVD$\downarrow$  & UCF FVD$\downarrow$  & \#Params  & \#Steps &  \\ \midrule
\multicolumn{5}{l}{\textit{Pixel-Space Generative Models}} \\
ARLM & Video Transformer~\citep{weissenborn2019scaling} & 170.0\mytiny{$\pm$5.0} & & 373M & 197k  \\
GAN & DVD-GAN-FP~\citep{clark2019adversarial}  & 69.1\mytiny{$\pm$1.2} & & & 1                    \\
GAN & TrIVD-GAN-FP~\citep{luc2020transformation}  & 25.7\mytiny{$\pm$0.7} &  & & 1                \\
Diffusion & RaMViD~\citep{hoppe2022diffusion}   &  17.5\mytiny{$\pm$1.1} & & 308M & 1000  \\
Diffusion & Video Diffusion~\citep{ho2022video}  & 16.2\mytiny{$\pm$0.3} & & 1.1B &   256        \\
Diffusion & RIN~\citep{jabri2023scalable} & 10.8 & & 411M & 1000 \\
\midrule
\multicolumn{6}{l}{\textit{Latent-Space Generative Models}} & Latent bpp\\
ARLM + VQ & LVT~\citep{rakhimov2021latent} & 224.7 &  & 50M  & 16k & 2.000 \\
ARLM + VQ & CogVideo$^*$~\citep{hong2022cogvideo}  & 109.2 & 626 & 9.4B   & 64k & 0.223$^*$        \\
ARLM + VQ & CCVS~\citep{le2021ccvs}   & 55.0\mytiny{$\pm$1.0} & 386\mytiny{$\pm$18} & 361M   & 1024& 0.219 \\
ARLM + VQ & TATS~\citep{ge2022long}  &  & 332\mytiny{$\pm$18} & 321M & 1024 &  0.055 \\
MLM + VQ & Phenaki~\citep{villegas2022phenaki} & 36.4\mytiny{$\pm$0.2} & & 227M   & 48 & 0.406\\
ARLM + DCT & Transframer~\citep{nash2022transframer}  & 25.4  &  & 662M &  $<$4k    & $\approx$6   \\
% T MAGVIT-B-FP        & 24.5\mytiny{$\pm$0.9}     & 43.3\mytiny{$\pm$1.8} & 88M & 0.039 & 12 \\
MLM + VQ & MAGVIT~\citep{yu2022magvit}        & 9.9\mytiny{$\pm$0.3} & 76\mytiny{$\pm$2} & 306M   & 12 & 0.039 \\ 
\hdashline
\multirow{2}{*}{MLM + \quantizername{}} & \multirow{2}{*}{\emph{\modelname{} (this paper)}} & 5.2\mytiny{$\pm$0.2} &  & \multirow{2}{*}{307M} & 12 & \multirow{2}{*}{0.070} \\
 & & \textbf{4.3\mytiny{$\pm$0.1}}  & \textbf{58\mytiny{$\pm$3}} & & 24 &  \\
\bottomrule
\end{tabular}
}
\end{subtable}

\begin{subtable}{\linewidth}
\vspace{2mm}
\caption{Class-conditional image generation on ImageNet 512$\times$512.
% \lu{we can remove GAN.} \lijun{recent diffusion papers all kept those, esp. StyleGAN-XL which is very strong}
}
\label{tab:gen_in512_full}
\vspace{-2mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l@{\hspace{5pt}}l@{\hspace{4pt}}c@{\hspace{2pt}}c@{\hspace{3pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{5pt}}c@{}}
\toprule
\multirow{2}{*}{Type}  & \multirow{2}{*}{Method}  & \multicolumn{2}{c}{w/o guidance} & \multicolumn{2}{c}{w/ guidance}  & \multirow{2}{*}{\#Params}  & \multirow{2}{*}{\#Steps} &  \\
& & FID$\downarrow$ & IS$\uparrow$ & FID$\downarrow$ & IS$\uparrow$ \\ \midrule
% \multicolumn{6}{l}{\textbf{512 $\times$ 512 resolution}} \\
\multicolumn{6}{l}{\textit{Pixel-Space Generative Models}} \\
% ADM & & 23.24 & 58.06 & 7.72 & 172.71 \\
Diffusion & ADM+Upsample~\citep{dhariwal2021diffusion}  & 9.96  & 121.8 & 3.85 & 221.7 & 731M & 2000 \\
GAN & BigGAN-deep~\citep{brock2018large} & 8.43 & 177.9 & & & 160M  & 1 \\
Diffusion & RIN~\citep{jabri2023scalable} & 3.95 & 216.0 & & & 320M  & 1000 \\
Diffusion & simple diffusion~\citep{hoogeboom2023simple} & 3.54 & 205.3 & 3.02 & 248.7 & 2B & 512 &\\
Diffusion & VDM++~\citep{kingma2023vdm}  & 2.99 & 232.2 & 2.65 & 278.1  & 2B & 512 \\
GAN & StyleGAN-XL~\citep{sauer2022stylegan} & & & 2.41 & 267.8 & 168M & 1 \\
\midrule
\multicolumn{8}{l}{\textit{Latent-Space Generative Models}} & Latent bpp \\
Diff. + VAE & DiT-XL/2~\citep{peebles2022scalable} & 12.03 & 105.3 & 3.04 & 240.8 & 675M  & 250 & 2.000$^*$ \\
 
MLM + VQ & MaskGIT~\citep{chang2022maskgit} & 7.32 & 156.0 & & & 227M & 12  & 0.039 \\
MLM + VQ & Token-Critic~\citep{lezama2022improved} & 6.80 & 182.1 &  &  & 368M & 36 & 0.039 \\
MLM + VQ & DPC+Upsample~\citep{lezama2022discrete}  & 3.62 & 249.4 & & & 619M & 72 & 0.039   \\
% MLM + VQ & DPC-light(5)+U~\citep{lezama2022discrete}  & 3.62 & 249.40 & & & 619M & 72 & 0.039   \\
\hdashline
\multirow{2}{*}{MLM + \quantizername{}} & \multirow{2}{*}{\emph{\modelname{} (this paper)}} & 4.61 & 192.4 & & & \multirow{2}{*}{307M} & 12 & \multirow{2}{*}{\textbf{0.018}} \\
& & 3.07 & 213.1 & \textbf{1.91} & \textbf{324.3} &  & 64 & \\
% & \emph{\modelname{} (this paper)} (40 bits) &  & & &  & 312M & & 0.039 \\
\bottomrule
\end{tabular}}
\end{subtable}

\end{table}

